Network Pruning Spaces

Network pruning techniques, including weight pruning and filter pruning, reveal that most state-of-the-art neural networks can be accelerated without a significant performance drop. This work focuses on filter pruning which enables accelerated inference with any off-the-shelf deep learning library and hardware. We propose the concept of \emph{network pruning spaces} that parametrize populations of subnetwork architectures. Based on this concept, we explore the structure aspect of subnetworks that result in minimal loss of accuracy in different pruning regimes and arrive at a series of observations by comparing subnetwork distributions. We conjecture through empirical studies that there exists an optimal FLOPs-to-parameter-bucket ratio related to the design of original network in a pruning regime. Statistically, the structure of a winning subnetwork guarantees an approximately optimal ratio in this regime. Upon our conjectures, we further refine the initial pruning space to reduce the cost of searching a good subnetwork architecture. Our experimental results on ImageNet show that the subnetwork we found is superior to those from the state-of-the-art pruning methods under comparable FLOPs.

==> backup/2_preliminaries.tex <==
\section{Preliminaries}

\subsection{Pruning filters}

We briefly describe filter pruning of convolutional layers.
Extending filter pruning to fully-connected layers is straightforward.
Let $c_i$ denote the number of input channels for the $i$th convolutional layer in a network and $h_i / w_i$ be the height/width of the input feature maps.
The convolutional layer transforms the input feature maps $x_i \in R^{c_i \times h_i \times w_i}$ into the output feature maps $x_{i + 1} \in R^{c_{i + 1} \times h_{i + 1} \times w_{i + 1}}$, which are used as input feature maps for the next convolutional layer.
This is achieved by applying $c_{i + 1}$ 3D filters $F_{i, j} \in R^{c_i \times h_i \times w_i}$ on the $c_i$ input channels, in which one filter generates one feature map.
Each filter is composed by $c_i$ 2D kernels $K \in R^{k \times k}$ (\eg, $3 \times 3$ and $1 \times 1$ in ResNet~\citep{he2016deep}).
All the filters, together, constitute the kernel matrix $F_i \in R^{c_i \times c_{i + 1} \times k \times k}$.
When a filter $F_{i, j}$ is pruned, its corresponding feature map $x_{i + 1, j}$ is removed.
The kernels that apply on the removed feature maps from filters of the next convolutional layer are also removed.
Pruning $m$ filters of layer $i$ will reduce $m / c_{i + 1}$ of the computation cost for both layers $i$ and $i + 1$.

For modern CNN architectures, pruning filters may not be straightforward.


==> backup/fig_f_params.tex <==
\begin{figure}[!t]
\centering
\begin{subfigure}[b]{0.325\linewidth}
\includegraphics[width=\linewidth]{figs/drop_params_ttt.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.325\linewidth}
\includegraphics[width=\linewidth]{figs/drop_budget_ttt.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.325\linewidth}
\includegraphics[width=\linewidth]{figs/flops_budget_ttt.png}
\end{subfigure}
%
\caption{
In this figure, we present the best 40 subnetworks on all \std spaces for each $c_{\textnormal{flops}}$.
(\emph{Left}) Parameter bucket distribution of winning subnetworks.
(\emph{Right}) Mean computation budget distribution of winning subnetworks.
}
\label{fig:f_params}
\end{figure}


==> backup/fig_p_flops.tex <==
\begin{figure}[!t]
\centering
\begin{subfigure}[b]{0.48\linewidth}
\includegraphics[width=\linewidth]{figs/drop_flops_ddd.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.48\linewidth}
\includegraphics[width=\linewidth]{figs/drop_budget_ddd.png}    
\end{subfigure}
%
\caption{
In this figure, we present the best 40 subnetworks on all \std spaces for each $c_{\textnormal{flops}}$.
(\emph{Left}) Parameter bucket distribution of winning subnetworks.
(\emph{Right}) Mean computation budget distribution of winning subnetworks.
}
\label{fig:p_flops}
\end{figure}


==> backup/fig_prune.tex <==
\begin{figure}[!t]
\centering
\begin{subtable}{0.45\textwidth}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lccc@{}}
\toprule
pruning    & pruning ratio & retraining epochs & Top-1$\downarrow$ (\%) \\
\midrule
one-shot   & 0.75   & 200  & $-0.5  \pm 0.23$ \\
iterative  & 0.75   & 1000 & $-0.48 \pm 0.15$ \\
\bottomrule
\end{tabular}
}
\end{subtable}
%
\begin{subfigure}{0.49\textwidth}
\centering
\includegraphics[width=\linewidth]{figs/filters.png}
\end{subfigure}
\caption{Filter pruning results on CIFAR-10.
(\emph{Left}) Comparison of uniform pruning ratios and pruning recipes from our \texttt{STD} pruning spaces.
(\emph{Right}) Pruning filters of ResNet-50 based on different pruning heuristics, including $\ell_1$ norm, $\ell_2$ norm and FPGM~\citep{he2019filter}.
}
\label{fig:prune}
\end{figure}

==> backup/fig_spaces_backup.tex <==
\begin{figure}[!t]
\centering
\begin{subfigure}[b]{\spacefigwidth\linewidth}
\includegraphics[width=\linewidth]{figs/edfs_f95.png}
\end{subfigure}
%
\begin{subfigure}[b]{\spacefigwidth\linewidth}
\includegraphics[width=\linewidth]{figs/drop_std_f95.png}
\end{subfigure}
%
\begin{subfigure}[b]{\spacefigwidth\linewidth}
\includegraphics[width=\linewidth]{figs/drop_flops_f95.png}
\end{subfigure}
%
\begin{subfigure}[b]{\spacefigwidth\linewidth}
\includegraphics[width=\linewidth]{figs/best_models_f95.png}
\end{subfigure}
\caption{Caption}
\label{fig:space95}
\end{figure}

\begin{figure}[!t]
\centering
\begin{subfigure}[b]{\spacefigwidth\linewidth}
\includegraphics[width=\linewidth]{figs/edfs_f75.png}
\end{subfigure}
%
\begin{subfigure}[b]{\spacefigwidth\linewidth}
\includegraphics[width=\linewidth]{figs/drop_std_f75.png}
\end{subfigure}
%
\begin{subfigure}[b]{\spacefigwidth\linewidth}
\includegraphics[width=\linewidth]{figs/drop_flops_f75.png}
\end{subfigure}
%
\begin{subfigure}[b]{\spacefigwidth\linewidth}
\includegraphics[width=\linewidth]{figs/best_models_f75.png}
\end{subfigure}
\caption{Caption}
\label{fig:space75}
\end{figure}

\def\spacefigwidth{0.49}
\begin{figure}[!t]
\centering
\begin{subfigure}[b]{\spacefigwidth\linewidth}
\includegraphics[width=\linewidth]{figs/edfs_f75.png}
\end{subfigure}
%
\begin{subfigure}[b]{\spacefigwidth\linewidth}
\includegraphics[width=\linewidth]{figs/edfs_f95.png}
\end{subfigure}
%
\begin{subfigure}[b]{\spacefigwidth\linewidth}
\includegraphics[width=\linewidth]{figs/drop_std_f75.png}
\end{subfigure}
%
\begin{subfigure}[b]{\spacefigwidth\linewidth}
\includegraphics[width=\linewidth]{figs/drop_std_f95.png}
\end{subfigure}
%
\begin{subfigure}[b]{\spacefigwidth\linewidth}
\includegraphics[width=\linewidth]{figs/drop_flops_f75.png}
\end{subfigure}
%
\begin{subfigure}[b]{\spacefigwidth\linewidth}
\includegraphics[width=\linewidth]{figs/drop_flops_f95.png}
\end{subfigure}
%
\begin{subfigure}[b]{\spacefigwidth\linewidth}
\includegraphics[width=\linewidth]{figs/best_models_f75.png}
\caption{$c_{\textnormal{flops}} = 0.25$}
\end{subfigure}
%
\begin{subfigure}[b]{\spacefigwidth\linewidth}
\includegraphics[width=\linewidth]{figs/best_models_f95.png}
\caption{$c_{\textnormal{flops}} = 0.05$}
\end{subfigure}
\caption{Network pruning spaces under $c_{\textnormal{flops}} = 0.25$ and $c_{\textnormal{flops}} = 0.05$.
}
\label{fig:spaces}
\end{figure}


==> backup/tab.tex <==
% \begin{table}[!t]
% \centering
% \caption{Filter pruning results with the proposed baseline setting.
% }
% \label{tab:baseline}
% % \resizebox{\linewidth}{!}{
% \begin{tabular}{@{}lcccccc@{}}
% \toprule
% network & dataset & $r$ & FLOPs (G) & $t$ & top-1 (\%) & accuracy drop (\%) \\
% \midrule
% ResNet-50 & CIFAR-10    & -     & 4.12 & -    & 95.88 & -     \\
% ResNet-50 & CIFAR-10    & 0.5   & 1.07 & 50   & 95.58 & 0.30  \\
% ResNet-50 & CIFAR-10    & 0.5   & 1.07 & 200  & 95.88 & 0.00  \\
% ResNet-50 & CIFAR-10    & 0.75  & 0.29 & 50   & 95.17 & 0.71  \\
% ResNet-50 & CIFAR-10    & 0.75  & 0.29 & 200  & 95.24 & 0.64  \\
% ResNet-50 & ImageNet    & -     & 4.12 & -   & 76.86 & -     \\
% ResNet-50 & ImageNet    & 0.75  & 0.29 & 50   & 61.76 & 15.10 \\
% ResNet-50 & ImageNet    & 0.75  & 0.29 & 100  & 61.76 & 15.10 \\
% \bottomrule
% \end{tabular}
% % }
% \end{table}


==> floats/fig_irregnet.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/edfs_ir95.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/drop_budget_ir95.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/best_models_ir95.png}
\end{subfigure}
%
\caption{Pruning IrRegNet-50 on \std spaces under $c_{\textnormal{flops}} = 0.05$.
(\emph{Left}) Accuracy drop EDFs on \texttt{STD} spaces.
(\emph{Center}) Mean computation budget distribution.
(\emph{Right}) The winning pruning recipe on each \std space.
}
\label{fig:irregnet}
\end{figure}


==> floats/fig_std_spaces_flops_mob_v2_cifar10.tex <==
\begin{figure}[!t]
\centering
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/flops_0.75_EDFs.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/flops_0.90_EDFs.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/flops_0.95_EDFs.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/flops_0.75_std_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/flops_0.90_std_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/flops_0.95_std_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/flops_0.75_flops_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/flops_0.90_flops_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/flops_0.95_flops_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/flops_0.75_params_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/flops_0.90_params_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/flops_0.95_params_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/flops_0.75_budget_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/flops_0.90_budget_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/flops_0.95_budget_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/flops_0.75_winning_recipes.png}
\caption{$c_{\textnormal{flops}} = 0.25$}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/flops_0.90_winning_recipes.png}
\caption{$c_{\textnormal{flops}} = 0.1$}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/flops_0.95_winning_recipes.png}
\caption{$c_{\textnormal{flops}} = 0.05$}
\end{subfigure}
%
\caption{
test.
}
\label{fig:std_spcaes_flops_mob_v2_cifar10}
\end{figure}


==> floats/fig_std_spaces_flops_r50_cifar10.tex <==
\begin{figure}[!t]
\centering
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/flops_0.75_EDFs.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/flops_0.90_EDFs.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/flops_0.95_EDFs.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/flops_0.75_std_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/flops_0.90_std_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/flops_0.95_std_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/flops_0.75_flops_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/flops_0.90_flops_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/flops_0.95_flops_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/flops_0.75_params_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/flops_0.90_params_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/flops_0.95_params_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/flops_0.75_budget_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/flops_0.90_budget_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/flops_0.95_budget_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/flops_0.75_winning_recipes.png}
\caption{$c_{\textnormal{flops}} = 0.25$}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/flops_0.90_winning_recipes.png}
\caption{$c_{\textnormal{flops}} = 0.1$}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/flops_0.95_winning_recipes.png}
\caption{$c_{\textnormal{flops}} = 0.05$}
\end{subfigure}
%
\caption{
test.
}
\label{fig:std_spcaes_flops_r50_cifar10}
\end{figure}


==> floats/fig_std_spaces_params_mob_v2_cifar10.tex <==
\begin{figure}[!t]
\centering
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/params_0.75_EDFs.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/params_0.90_EDFs.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/params_0.95_EDFs.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/params_0.75_std_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/params_0.90_std_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/params_0.95_std_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/params_0.75_flops_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/params_0.90_flops_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/params_0.95_flops_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/params_0.75_params_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/params_0.90_params_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/params_0.95_params_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/params_0.75_budget_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/params_0.90_budget_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/params_0.95_budget_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/params_0.75_winning_recipes.png}
\caption{$c_{\textnormal{params}} = 0.25$}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/params_0.90_winning_recipes.png}
\caption{$c_{\textnormal{params}} = 0.1$}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/mob_v2_cifar10/params_0.95_winning_recipes.png}
\caption{$c_{\textnormal{params}} = 0.05$}
\end{subfigure}
%
\caption{
test.
}
\label{fig:std_spcaes_params_mob_v2_cifar10}
\end{figure}


==> floats/fig_std_spaces_params_r50_cifar10.tex <==
\begin{figure}[!t]
\centering
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/params_0.75_EDFs.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/params_0.90_EDFs.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/params_0.95_EDFs.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/params_0.75_std_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/params_0.90_std_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/params_0.95_std_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/params_0.75_flops_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/params_0.90_flops_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/params_0.95_flops_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/params_0.75_params_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/params_0.90_params_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/params_0.95_params_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/params_0.75_budget_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/params_0.90_budget_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/params_0.95_budget_to_drop.png}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/params_0.75_winning_recipes.png}
\caption{$c_{\textnormal{params}} = 0.25$}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/params_0.90_winning_recipes.png}
\caption{$c_{\textnormal{params}} = 0.1$}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{figs/r50_cifar10/params_0.95_winning_recipes.png}
\caption{$c_{\textnormal{params}} = 0.05$}
\end{subfigure}
%
\caption{
test.
}
\label{fig:std_spcaes_params_r50_cifar10}
\end{figure}


==> parts/s_related_work.tex <==
\section{Related work}

In this section, we discuss some related works.

